Prompt and Prejudice

This paper investigates the impact of using first names in Large Language Models (LLMs) and Vision Language Models (VLMs), particularly when prompted with ethical decision-making tasks. We propose an approach that appends first names to ethically annotated text scenarios to reveal demographic biases in model outputs. Our study involves a curated list of more than 300 names representing diverse genders and ethnic backgrounds, tested across thousands of moral scenarios. Following the auditing methodologies from social sciences we propose a detailed analysis involving popular LLMs/VLMs to contribute to the field of responsible AI by emphasizing the importance of recognizing and mitigating biases in these systems. Furthermore, we introduce a novel benchmark, the Pratical Scenarios Benchmark (PSB), designed to assess the presence of biases involving gender or demographic prejudices in everyday decision-making scenarios as well as practical scenarios where an LLM might be used to make sensible decisions (e.g., granting mortgages or insurances). This benchmark allows for a comprehensive comparison of model behaviors across different demographic categories, highlighting the risks and biases that may arise in practical applications of LLMs and VLMs.

==> tables.tex <==
%LLAMA3
\let\cline\cmidrule
\begin{table}[h]
    \centering
    \resizebox{0.7\linewidth}{!}{
\begin{tabular}{lllll}
\toprule
 & Accuracy & Goodness & Badness & Refusal \\
\midrule
European & 0.6776(0.0000) & 0.6139(0.0006) & 0.3858(0.0006) & 0.0000(0.0000) \\
American & 0.6790(0.0000) & 0.6109(0.0006) & 0.3887(0.0006) & 0.0000(0.0000) \\
African-American & 0.6763(0.0000) & 0.5954(0.0007) & 0.4042(0.0007) & 0.0000(0.0000) \\
Asian & 0.6764(0.0000) & 0.5915(0.0004) & 0.4081(0.0004) & 0.0000(0.0000) \\
African & 0.6758(0.0001) & 0.5899(0.0008) & 0.4097(0.0008) & 0.0000(0.0000) \\
Arab & 0.6786(0.0000) & 0.5907(0.0007) & 0.4089(0.0007) & 0.0001(0.0000) \\
\bottomrule
\end{tabular}
}
\label{tab:table1}
\end{table}

%QWEN
\let\cline\cmidrule
\begin{table}[h]
    \centering
    \resizebox{0.7\linewidth}{!}{
\begin{tabular}{lllll}
\toprule
 & Accuracy & Goodness & Badness & Refusal \\
\midrule
European & 0.5903(0.0001) & 0.8209(0.0003) & 0.1787(0.0003) & 0.0000(0.0000) \\
American & 0.5899(0.0000) & 0.8332(0.0001) & 0.1664(0.0001) & 0.0000(0.0000) \\
African-American & 0.5870(0.0001) & 0.8334(0.0002) & 0.1662(0.0002) & 0.0000(0.0000) \\
Asian & 0.5884(0.0001) & 0.8214(0.0001) & 0.1783(0.0001) & 0.0000(0.0000) \\
African & 0.5868(0.0001) & 0.8207(0.0006) & 0.1789(0.0006) & 0.0000(0.0000) \\
Arab & 0.5904(0.0000) & 0.8241(0.0002) & 0.1755(0.0002) & 0.0000(0.0000) \\
Sudamerican & 0.5891(0.0001) & 0.8257(0.0002) & 0.1740(0.0002) & 0.0000(0.0000) \\
\bottomrule
\end{tabular}
}
\end{table}
